Building the perfect game -- an empirical study of game modifications

Game developers cannot always meet the growing and changing needs of the gaming community, due to the often already overloaded schedules of developers. So-called modders can potentially assist game developers with addressing gamers' needs. Modders are enthusiasts who provide modifications or completely new content for a game. By supporting modders, game developers can meet the rapidly growing and varying needs of their gamer base. Modders have the potential to play a role in extending the life expectancy of a game, thereby saving game developers time and money, and leading to a better overall gaming experience for their gamer base. In this paper, we empirically study the metadata of 9,521 mods of the 20 most-modded games on the Nexus Mods distribution platform. Our goal is to provide useful insights into the modding community of the Nexus Mods distribution platform from a quantitative perspective, and to provide researchers with a solid foundation for future exploration of game mods. In doing so, game developers can potentially reduce development time and cost due to the increased replayability of their games through mods. We find that providing official support for mods can be beneficial for the perceived quality of the mods of a game. In addition, mod users are willing to submit bug reports for a mod. However, they often fail to do this in a systematic manner using the bug reporting tool of the Nexus Mods platform, resulting in low-quality bug reports which are difficult to resolve. Based on our findings, we recommend that game developers who desire an active modding community for their own games provide the modding community with an officially-supported modding tool. In addition, we recommend that mod distribution platforms, such as Nexus Mods, improve their bug reporting system to receive higher quality bug reports.

==> sections/discussion.tex <==
\section{Discussion}
\label{discuss}

In this section, we discuss two observations we have during the analysis, which can point to future works.

\subsection{Emergent updates within 24 hours}

As can be seen from Figure~\ref{how_many_hotfix} in RQ1, the percentage of self-admitted hotfixes are lower than 24 hours hotfixes, indicating that there are many updates pushed within 24 hours after previous adjacent updates, which are not recognized by developers to be hotfixes. We defined these updates as self-denied hotfixes. In general, 572 out of 600 24hr hotfixes are self-denied hotfixes. Figure~\ref{self_deny} shows the distribution of self-denied hotfixes.

\begin{figure}[h!]
  \centering
    \includegraphics[width=\columnwidth]{img/discussion/self_deny}
  \caption{Distribution of \# of self-denied hotfixes / \# of 24hr hotfixes}
  \label{self_deny}
\end{figure}

As can be seen from the figure, the majority of studied games have a ratio of self-denied hotfixes to 24hr hotfixes higher than 90\%. 

We look into the two outliers with a ratio of 20\% and 44\%. The outlier with a ratio of 20\% is the game \emph{DayZ} which has five 24hr hotfixes in total and one self-denied hotfix released on Dec 18, 2013. The developers mentioned the self-denied one contains "Various critical security updates". Considering Table~\ref{delay_reason} in RQ3 shows that Security has the lowest ratio of slow hotfixes to total hotfixes, we think although developers described the release note in the same way as an usual product update, it actually is a hotfix.

The other outlier with a ratio of 44\%, the game \emph{7 Days to Die}, has a different case. The game has nine 24hr hotfixes, among which four are self-denied. We find that the developers for this game use multiple phrase like "hot fix", "quick fix" and "patch" to describe hotfixes, hence we didn't match some 24hr hotfixes as self-admitted hotfixes with our regular expression. However, patch usually refers to a bigger concept than hotfix without specifying the emergency as the concept hotfix does. Hence we consider the developers misuse the term patch.

The high percentage of self-denied hotfixes is well worth studying. Future work can focus on other reasons causing self-denied hotfixes.

\subsection{The effect of hotfixes on game activity}

In this section, we do a preliminary study to identify the unusual activity drop of games, in order to try to quantify the effect of the number of days it takes to release a hotfix on the number of players.

\subsubsection{Unusual Activity Drop}

As mentioned in Section~\ref{method}, we use number of players as the metric for quantifying activities of games. Hence the Unusual Activity Drop (UAD) of games actually means the dates with unusual drop on the number of players.


% --------------NEED TO BE REWRITE!!-------------
We hereby propose an approach to identify the UAD of games. The approach use different threshold for each weekday. For example, when identifying all the Mondays containing UAD, we firstly calculate the difference of numbers of players between the Sundays and the following Mondays, divided by the numbers of players on the first Sunday. Secondly we calculated the mean and standard deviation of these values. Then for each (Sunday - Monday) / Sunday, we compared the value with the mean value - 2 * standard deviation. If the drop is greater than two times standard deviation, we identified an UAD happened on that Monday.
% -------------------------------------------------------------

The approach can avoid the influence of two kinds of fluctuation of numbers of players we mentioned on Section~\ref{method}.

\subsubsection{Relation between the time it takes for releasing hotfixes and UAD}

After applying the above mentioned UAD identification approach to all the studied games, we have a list of dates with UAD for each game. We then count the number of UAD happens between each hotfix and its previous adjacent update. We classify the hotfixes by whether or not they have UAD before their release. Figure~\ref{compareuad} compares the distribution of days between hotfixes and previous adjacent product updates for these two classes of hotfixes. In order to better demonstrate the distribution, we remove two outliers with values of 169 and 394 days, both of which have at least 1 UAD.

\begin{figure}[h!]
  \centering
    \includegraphics[width=\columnwidth]{img/discussion/UADvsDelay}
  \caption{Delay comparison of two classes of hotfixes}
  \label{compareuad}
\end{figure}

To better understand the relation, we plot Figure~\ref{scatterplot} to show the relation between the days it takes for releasing hotfixes and the count of UAD. Each point in the figure represents a hotfix while the line is a smooth curve computed by local polynomial regression fitting using 1 degree of polynomial. For a better demonstration, we remove a outlying point (394, 68) which also agree with the trend. 

\begin{figure}[h!]
  \centering
    \includegraphics[width=\columnwidth]{img/discussion/scatterplot}
  \caption{Relation between days between hotfixes and previous product updates and count of UAD}
  \label{scatterplot}
\end{figure}

For comparison, we also generate the scatterplot and smooth curve for regular product updates using the same algorithm and range, as shown in Figure~\ref{scatterplot_regular_update}. The slope of curve for regular product updates is lower than that for hotfixes, as 991 of 1328 (75\%) points in Figure~\ref{scatterplot_regular_update} have a count of UAD of 0. Figure~\ref{scatterplot} and Figure~\ref{scatterplot_regular_update} indicate that the longer it takes to release hotfixes, the more likely that the game would suffer a unusual activity drop.

\begin{figure}[h!]
  \centering
    \includegraphics[width=\columnwidth]{img/discussion/scatterplot_regular_update}
  \caption{Relation between days between adjacent product updates and count of UAD}
  \label{scatterplot_regular_update}
\end{figure}

To verify this observation, we calculate the Spearman's correlation between count of UAD and the time for releasing hotfixes and regular product updates respectively. The Spearman's $\rho$ score for count of UAD and days between hotfixes and previous updates is 0.86, while the Spearman's $\rho$ score for count of UAD and days between adjacent regular product updates is -0.01. The Spearman's correlation test shows a significant correlation between the time it takes for releasing hotfixes and the appearance of UAD, while the regular product updates do not.

\subsubsection{The most common reasons for hotfixes suffering UAD}

We also look at the rank of reasons causing hotfixes with UAD, as it might reflect the emergency of reasons from users' perspective. The result is shown in Table~\ref{uadreason}.

\begin{table} [h!]
	\centering
	\caption{Rank of Reasons for hotfixes with UAD} 
	\label{uadreason}
	\resizebox{0.84\columnwidth}{!}{  
	\begin{tabular} { c | c | c }
	\hline
	\bfseries Reason & \bfseries \# of hotfixes & \bfseries Percentage  \\ \hline \hline
	Functionality	 & 12 	& 28\% \\ \hline
	Visual		 & 11 	& 26\% \\ \hline
	Rule			 & 5	 	& 12\% \\ \hline
	Balance		 & 5	 	& 12\% \\ \hline
	Performance	 & 5	 	& 12\% \\ \hline
	Crash		 & 4	 	& 9\% \\ \hline
	Content		 & 4	 	& 9\% \\ \hline
	UI			 & 3	 	& 7\% \\ \hline
	Sound		 & 3	 	& 7\%  \\ \hline
	Localization	 & 1	 	& 2\% \\ \hline
	Security		 & 0	 	& 0\% \\ \hline
	Desync		 & 0	 	& 0\% \\ \hline
	\hline
	\end{tabular}}
\end{table}

As Table~\ref{uadreason} shows, games with problems regarding Functionality and Visual are more likely to suffer an unusual activity drop, indicating that game players are more sensitive with Functionality and Visual problems while less sensitive with Localization, Security and Desync problems. However from the findings of RQ3, we see that Functionality and Visual are both not time-sensitive from developers' perspective. This observation may help developers learn about their customers better, and adjust the update strategy to best meet players' requirements by raising the priority of Functionality and Visual issues.

